Should Audio Front-ends be Adaptive? Comparing Learnable and Adaptive Front-ends

Hand-crafted features, such as Mel-filterbanks, have traditionally been the choice for many audio processing applications. Recently, there has been a growing interest in learnable front-ends that extract representations directly from the raw audio waveform. \textcolor{black}{However, both hand-crafted filterbanks and current learnable front-ends lead to fixed computation graphs at inference time, failing to dynamically adapt to varying acoustic environments, a key feature of human auditory systems.} To this end, we explore the question of whether audio front-ends should be adaptive by comparing the Ada-FE front-end (a recently developed adaptive front-end that employs a neural adaptive feedback controller to dynamically adjust the Q-factors of its spectral decomposition filters) to established learnable front-ends. Specifically, we systematically investigate learnable front-ends and Ada-FE across two commonly used back-end backbones and a wide range of audio benchmarks including speech, sound event, and music. The comprehensive results show that our Ada-FE outperforms advanced learnable front-ends, and more importantly, it exhibits impressive stability or robustness on test samples over various training epochs.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> TFA.tex <==
\begin{table*}[!t]
\centering
    % \scriptsize
    % \footnotesize
    \small
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.3pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
\caption{\textcolor{blue}{The results of SincNet and SincNet with dynamic time-frequency attention.}}
% \vspace*{-0.5em}
% \scalebox{1}{
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
\toprule
% \hline
% Task & Acoustic Scene & \multicolumn{2}{c|}{Music Genre} & \multicolumn{2}{c|}{Speech Emotion} & \multicolumn{2}{c|}{keyword Spotting} & Speaker Id. \\
% \hline
Task & \multirow{2}{*}{Back-end} & \multicolumn{2}{c|}{ESC-50} & \multicolumn{2}{c|}{GTZAN} &  \multicolumn{2}{c|}{FMA-Small} & \multicolumn{2}{c|}{CREMA-D} & \multicolumn{2}{c|}{SPC-V1} & \multicolumn{2}{c}{SPC-V2} \\
% \hline
\cline{3-14}
Accuracy & & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
% \hline
% Segment & -- & -- & -- & -- & -- & -- & -- & 1 s & 3 s \\
\hline
\hline
SincNet & \multirow{2}{*}{ENet-B0} &
\textcolor{black}{64.80} & \textcolor{black}{88.00} & \textcolor{blue}{51.38} & \textcolor{blue}{94.83} & \textcolor{blue}{50.00} & \textcolor{blue}{94.75} & \textcolor{blue}{53.43} & \textcolor{blue}{98.07} & \textcolor{black}{61.61} & \textcolor{black}{89.34} & \textcolor{black}{68.44} & \textcolor{black}{89.22} \\

SincNet+TFA & & 
\textbf{\textcolor{black}{65.30}}  & \textcolor{black}{88.05} & \textcolor{blue}{51.72}  & \textcolor{blue}{94.83} & \textcolor{blue}{51.00} & \textcolor{blue}{95.38} & \textcolor{blue}{56.61} & \textcolor{blue}{99.23} & \textcolor{black}{62.94}  &  \textcolor{black}{85.33}  & \textcolor{black}{59.16} & \textcolor{black}{81.52} \\



\toprule
% \hline
% \rowcolor{orange!20} \,\,\,\,\, Fixed Gabor filter+AFC-Energy+FM & -- & -- & 54.14 & 95.52 & 45.38 & 93.63 & 59.78 & 98.84 & 91.92 & 98.19 \\
\end{tabular}
\label{ablation}
% }
\end{table*}

==> cbak.tex <==
\begin{table}[!ht]
    \centering
    \scriptsize
    \def\arraystretch{0.99}
    \setlength{\tabcolsep}{5.5pt}
    % \footnotesize	
    \caption{Average CBAK scores for each SNR condition and the highest CBAK scores are highlighted in boldface.}
    \label{tab:cbak}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||ccccc@{}}
        \hline
        &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cline{3-7}
        Objective & Network & -5 & 0 & 5 & 10 & 15 \\
        \hline
        - & Noisy & 1.15 & 1.40 & 1.58 & 2.13 & 2.61 \\
        \hline
        \hline
        \multirow{8}{*}{IRM}
        & ResTCN & 1.69 & 2.03 & 2.41 & 2.85 & 3.30 \\
        & +FA    & 1.75 & 2.10 & 2.50 & 2.94 & 3.39 \\
        & +TA    & 1.74 & 2.09 & 2.51 & 2.95 & 3.38 \\
        & +TFA   & \textbf{1.79} & \textbf{2.15} & \textbf{2.56} & \textbf{2.99} & \textbf{3.42} \\
        \cline{2-7}
        & MHANet & 1.69 & 2.03 & 2.43 & 2.86 & 3.31 \\
        & +FA    & 1.75 & 2.10 & 2.50 & 2.93 & 3.36 \\
        & +TA    & 1.73 & 2.10 & 2.50 & 2.94 & 3.37 \\
        & +TFA   & \textbf{1.79} & \textbf{2.14} & \textbf{2.55} & \textbf{2.98} & \textbf{3.42} \\
        \hline
        \hline
        
        \multirow{8}{*}{SMM}
        & ResTCN & 1.71 & 2.04 & 2.41 & 2.81 & 3.23\\
        & +FA    & 1.78 & 2.14 & 2.53 & 2.96 & 3.39\\
        & +TA    & 1.77 & 2.13 & 2.53 & 2.96 & 3.39\\
        & +TFA   & \textbf{1.85} & \textbf{2.21} & \textbf{2.60} & \textbf{3.04} & \textbf{3.46} \\
        \cline{2-7}
        & MHANet & 1.72 & 2.07 & 2.46 & 2.89 & 3.34 \\
        & +FA    & 1.77 & 2.14 & 2.54 & 2.97 & 3.39 \\
        & +TA    & 1.80 & 2.16 & 2.56 & 2.94 & 3.41\\
        & +TFA   & \textbf{1.83} & \textbf{2.20} & \textbf{2.60} & \textbf{3.03} & \textbf{3.45} \\
        \hline
        \hline
        
        \multirow{8}{*}{PSM}
        & ResTCN & 1.70 & 2.07 & 2.49 & 2.94 & 3.41 \\
        & +FA    & 1.78 & 2.15 & 2.58 & 3.03 & 3.49 \\
        & +TA    & 1.73 & 2.12 & 2.55 & 3.01 & 3.46 \\
        & +TFA   & \textbf{1.80} & \textbf{2.19} & \textbf{2.62} & \textbf{3.08} & \textbf{3.53} \\
        \cline{2-7}
        & MHANet & 1.60 & 2.08 & 2.51 & 2.98 & 3.44 \\
        & +FA    & 1.78 & 2.15 & 2.57 & 3.02 & 3.48 \\
        & +TA    & 1.75 & 2.13 & 2.56 & 3.02 & 3.48 \\
        & +TFA   & \textbf{1.80} & \textbf{2.19} & \textbf{2.61} & \textbf{3.06} & \textbf{3.49} \\
        \hline
        \hline
        
        \multirow{8}{*}{Xi}
        & ResTCN & 1.75 & 2.11 & 2.50 & 2.95 & 3.39 \\
        & +FA    & 1.85 & 2.21 & 2.61 & 3.06 & 3.50 \\
        & +TA    & 1.85 & 2.21 & 2.61 & 3.05 & 3.49 \\
        & +TFA   & \textbf{1.90} & \textbf{2.26} & \textbf{2.67} & \textbf{3.11} & \textbf{3.53} \\
        \cline{2-7}
        & MHANet & 1.78 & 2.15 & 2.50 & 3.01 & 3.46 \\
        & +FA    & 1.85 & 2.21 & 2.52 & 3.06 & 3.50 \\
        & +TA    & 1.82 & 2.19 & 2.54 & 3.04 & 3.47 \\
        & +TFA   & \textbf{1.88} & \textbf{2.24} & \textbf{2.59} & \textbf{3.09} & \textbf{3.51}\\
        \hline
    \end{tabular}
    \vspace{-2.0em}
\end{table}

==> covl.tex <==
\begin{table}[!h]
    \centering
    \scriptsize
    \def\arraystretch{0.99}
    \setlength{\tabcolsep}{5.5pt}
    % \footnotesize	
    \caption{Average COVL scores for each SNR condition and the highest COVL scores are highlighted in boldface.}
    \label{tab:covl}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||ccccc@{}}
        \hline
        &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cline{3-7}
        Objective & Network & -5 & 0 & 5 & 10 & 15 \\
        \hline
        - & Noisy & 1.17 & 1.32 & 1.58 & 1.92 & 2.37 \\
        \hline
        \hline
        \multirow{8}{*}{IRM}
        & ResTCN & 1.56 & 1.94 & 2.34 & 2.81 & 3.26 \\
        & +FA    & 1.66 & 2.04 & 2.47 & 2.94 & 3.40 \\
        & +TA    & 1.65 & 2.04 & 2.48 & 2.95 & 3.37 \\
        & +TFA   & \textbf{1.73} & \textbf{2.15} & \textbf{2.57} & \textbf{2.99} & \textbf{3.45} \\
        \cline{2-7}
        & MHANet & 1.58 & 1.95 & 2.39 & 2.84 & 3.30 \\
        & +FA    & 1.64 & 2.02 & 2.45 & 2.92 & 3.36 \\
        & +TA    & 1.67 & 2.07 & 2.49 & 2.94 & 3.38 \\
        & +TFA   & \textbf{1.70} & \textbf{2.09} & \textbf{2.53} & \textbf{3.00} & \textbf{3.44} \\
        \hline
        \hline
        
        \multirow{8}{*}{SMM}
        & ResTCN & 1.53 & 1.90 & 2.30 & 2.75 & 3.19 \\
        & +FA    & 1.66 & 2.06 & 2.49 & 2.96 & 3.41 \\
        & +TA    & 1.65 & 2.06 & 2.50 & 2.97 & 3.41 \\
        & +TFA   & \textbf{1.72} & \textbf{2.15} & \textbf{2.60} & \textbf{3.06} & \textbf{3.49} \\
        \cline{2-7}
        & MHANet & 1.59 & 1.97 & 2.39 & 2.89 & 3.31 \\
        & +FA    & 1.64 & 2.03 & 2.48 & 2.97 & 3.37 \\
        & +TA    & 1.67 & 2.08 & 2.52 & 2.98 & 3.42 \\
        & +TFA   & \textbf{1.70} & \textbf{2.12} & \textbf{2.57} & \textbf{3.03} & \textbf{3.46} \\
        \hline
        \hline
        
        \multirow{8}{*}{PSM}
        & ResTCN & 1.55 & 1.95 & 2.40 & 2.89 & 3.38 \\
        & +FA    & 1.66 & 2.06 & 2.52 & 3.03 & 3.51 \\
        & +TA    & 1.64 & 2.08 & 2.55 & 3.05 & 3.51 \\
        & +TFA   & \textbf{1.72} & \textbf{2.14} & \textbf{2.62} & \textbf{3.10} & \textbf{3.55} \\
        \cline{2-7}
        & MHANet & 1.60 & 2.02 & 2.49 & 3.00 & 3.47 \\
        & +FA    & 1.65 & 2.06 & 2.53 & 3.03 & 3.51 \\
        & +TA    & 1.65 & 2.07 & 2.54 & 3.05 & 3.53 \\
        & +TFA   & \textbf{1.70} & \textbf{2.12} & \textbf{2.60} & \textbf{3.11} & \textbf{3.55} \\
        \hline
        \hline
        
        \multirow{8}{*}{Xi}
        & ResTCN & 1.59 & 1.99 & 2.40 & 2.89 & 3.34 \\
        & +FA    & 1.68 & 2.08 & 2.53 & 3.05 & 3.51 \\
        & +TA    & 1.67 & 2.09 & 2.54 & 3.03 & 3.49 \\
        & +TFA   & \textbf{1.76} & \textbf{2.18} & \textbf{2.63} & \textbf{3.13} & \textbf{3.53}  \\
        \cline{2-7}
        & MHANet & 1.63 & 2.05 & 2.50 & 3.00 & 3.47\\
        & +FA    & 1.69 & 2.10 & 2.52 & 3.04 & 3.50\\
        & +TA    & 1.68 & 2.10 & 2.54 & 3.03 & 3.48\\
        & +TFA   & \textbf{1.72} & \textbf{2.13} & \textbf{2.59} & \textbf{3.08} & \textbf{3.51} \\
        \hline
        
    \end{tabular}
    \vspace{-0.8em}
\end{table}

==> csig.tex <==
\begin{table}[!htbp]
    \centering
    \scriptsize
    \def\arraystretch{0.99}
    \setlength{\tabcolsep}{5.5pt}
    % \footnotesize	
    \caption{Average CSIG scores for each SNR level and the highest CSIG scores are highlighted in boldface.}
    \label{tab:csig}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||ccccc@{}}
        \hline
        &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cline{3-7}
        Objective & Network & -5 & 0 & 5 & 10 & 15 \\
        \hline
        - & Noisy & 1.49 & 1.80 & 2.20 & 2.65 & 3.16 \\
        \hline
        \hline
        \multirow{8}{*}{IRM}
        & ResTCN & 2.17 & 2.66 & 3.12 & 3.58 & 4.00  \\
        & +FA    & 2.33 & 2.80 & 3.26 & 3.71 & 4.13  \\
        & +TA    & 2.30 & 2.79 & 3.26 & 3.71 & 4.11 \\
        & +TFA   & \textbf{2.40} & \textbf{2.88} & \textbf{3.35} & \textbf{3.78} & \textbf{4.17}\\
        \cline{2-7}
        & MHANet & 2.20 & 2.68 & 3.17 & 3.63 & 4.05  \\
        & +FA & 2.29 & 2.76 & 3.23 & 3.69 & 4.10  \\
        & +TA & 2.33 & 2.83 & 3.28 & 3.72 & 4.12 \\
        & +TFA & \textbf{2.37} & \textbf{2.85} & \textbf{3.32} & \textbf{3.77} & \textbf{4.18}\\
        \hline
        \hline
        
        \multirow{8}{*}{SMM}
        & ResTCN & 2.10 & 2.59 & 3.06 & 3.51 & 3.94\\
        & +FA    & 2.30 & 2.80 & 3.27 & 3.73 & 4.14\\
        & +TA    & 2.29 & 2.80 & 3.28 & 3.74 & 4.14\\
        & +TFA   & \textbf{2.37} & \textbf{2.90} & \textbf{3.37} & \textbf{3.81} & \textbf{4.20}\\
        \cline{2-7}
        & MHANet & 2.21 & 2.70 & 3.17 & 3.63 & 4.06 \\
        & +FA    & 2.27 & 2.76 & 3.24 & 3.69 & 4.10 \\
        & +TA    & 2.30 & 2.81 & 3.29 & 3.74 & 4.15 \\
        & +TFA   & \textbf{2.36} & \textbf{2.86} & \textbf{3.34} & \textbf{3.78} & \textbf{4.18}\\
        \hline
        \hline
        
        \multirow{8}{*}{PSM}
        & ResTCN & 2.15 & 2.65 & 3.13 & 3.61 & 4.06 \\
        & +FA    & 2.30 & 2.78 & 3.26 & 3.74 & 4.18 \\
        & +TA    & 2.29 & 2.81 & 3.30 & 3.77 & 4.20 \\
        & +TFA   & \textbf{2.38} & \textbf{2.88} & \textbf{3.36} & \textbf{3.80} & \textbf{4.21} \\
        \cline{2-7}
        & MHANet & 2.22 & 2.73 & 3.23 & 3.73 & 4.16 \\
        & +FA    & 2.29 & 2.78 & 3.28 & 3.76 & 4.19 \\
        & +TA    & 2.30 & 2.80 & 3.30 & 3.78 & 4.22 \\
        & +TFA   & \textbf{2.36} & \textbf{2.86} & \textbf{3.35} & \textbf{3.82} & \textbf{4.23} \\
        \hline
        \hline
        
        \multirow{8}{*}{Xi}
        & ResTCN & 2.19 & 2.70 & 3.16 & 3.63 & 4.05 \\
        & +FA    & 2.32 & 2.79 & 3.27 & 3.76 & 4.19 \\
        & +TA    & 2.29 & 2.80 & 3.28 & 3.75 & 4.18 \\
        & +TFA   & \textbf{2.41} & \textbf{2.91} & \textbf{3.37} & \textbf{3.84} & \textbf{4.23} \\
        \cline{2-7}
        & MHANet & 2.26 & 2.77 & 3.25 & 3.72 & 4.16\\
        & +FA    & 2.33 & 2.82 & 3.27 & 3.75 & \textbf{4.18} \\
        & +TA    & 2.31 & 2.83 & 3.30 & 3.76 & 4.17\\
        & +TFA   & \textbf{2.37} & \textbf{2.86} & \textbf{3.34} & \textbf{3.79} & \textbf{4.18} \\
        \hline
    \end{tabular}
    \vspace{-0.8em}
\end{table}

==> demand.tex <==
% \renewcommand\arraystretch{1.0}
\begin{table}[!htbp]
\centering
    \scriptsize
    \def\arraystretch{0.98}
    \setlength{\tabcolsep}{1.0pt}
\caption{Comparison to multiple speech enhancement systems on the VoiceBank-DEMAND dataset. The highest scores are highlighted in boldface.}
% \vspace*{0.1in}
\scalebox{1.2}{
\begin{tabular}{l||c||ccccc }
\hline
\textbf{Method}  & \# \textbf{Param.} & \textbf{PESQ} & \textbf{STOI} (\%) & \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} \\
\hline 
Noisy & - & 1.97 & 92 & 3.35 & 2.44 & 2.63 \\
\hline 
\hline
SEGAN \cite{SEGAN} & 43.2M       
& 2.16 & 93 & 3.48 & 2.94 & 2.80  \\
\textcolor{black}{DSEGAN \cite{DSEGAN}} & --       
& 2.35 & 93 & 3.55 & 3.10 & 2.93  \\
% \textcolor{blue}{Wave-U-Net \cite{}} & 10.2M       
% & 2.40 & -- & 3.52 & 3.24 & 2.96  \\
MetricGAN \cite{metricgan} & 1.89M   
& 2.86 & -- & 3.99 & 3.18 & 3.42  \\
PHASEN \cite{phasen} & 8.41M   
& 2.99 & -- & 4.21 & 3.55 & 3.62  \\
TFT-Net \cite{tftnet} & --   
& 2.75 & -- & 3.93 & 3.44 & 3.34  \\
T-GSA \cite{mha_se} & --   
& 3.06 & -- & 4.18 & \textbf{3.59} & 3.62  \\
\textcolor{black}{WaveCRN \cite{wavecrn}} & 4.66M   
& 2.64 & -- & 3.94 & 3.37 & 3.29  \\
\textcolor{black}{DCCRN \cite{dccrn}} & 3.7M   
& 2.68 & 93.5 & 3.88 & 3.18 & 3.27  \\
DCCRN+ \cite{dccrn+}& 3.3M   
& 2.84 & -- & -- & -- & --  \\
\textcolor{black}{S-DCCRN \cite{sdccrn}} & 2.34M   
& 2.84 & 94 & 4.03 & 2.97 & 3.43  \\
DEMCUS \cite{demcus} & 58M  
& 3.07 & 95 & 4.31 & 3.40 & 3.63  \\
\textcolor{black}{MHSA+SPK \cite{koizumi2020speech}} & -- 
& 2.99 & -- & 4.15 & 3.42 & 3.57 \\
\textcolor{black}{HiFi-GAN \cite{hifigan}} & -- 
& 2.94 & -- & 4.07 & 3.07 & 3.49 \\
\textcolor{black}{SADNUNet \cite{sadnunet}} & 2.63M 
& 2.82 & 95 & 4.18 & 3.47 & 3.51 \\
\textcolor{black}{CTS-Net \cite{ctsnet}} & 4.35M 
& 2.94 & 94.7 & 4.26 & 3.45 & 3.59 \\
\textcolor{black}{DCTCN \cite{dctcn}} & 9.7M 
& 2.83 & -- & 3.91 & 3.37 & 3.37 \\
% \textcolor{blue}{PERL \cite{perl}} & 3.5M 
% & \textbf{3.15} & 95 & 4.18 & \textbf{3.60} & 3.67 \\
\textcolor{black}{CleanUNet \cite{cleanunet}} & 46.07M 
& 2.91 & \textbf{95.6} & \textbf{4.34} & 3.42 & 3.65 \\
SA-TCN \cite{sa-tcn} & 3.76M   
& 2.99 & 94.22 & 4.25 & 3.45 & 3.62  \\
MetricGAN+ \cite{metricgan+} & --   
& \textbf{3.15} & -- & 4.14 & 3.16 & 3.64  \\
SEAMNET\cite{seamnet} & 5.1M   
& -- & -- & 3.87 & 3.16 & 3.23  \\
ResTCN+TFA-Xi & 1.98M   
& 3.02 & 94.15 & 4.32 & 3.52 & \textbf{3.68}  \\
\hline  
\end{tabular}}
\label{demand}
\vspace{-2.0em}
\end{table}

==> eval_size.tex <==
% \renewcommand\arraystretch{1.0}
\begin{table}[!htbp]
\centering
    \scriptsize
    \def\arraystretch{0.98}
    \setlength{\tabcolsep}{1.0pt}
\caption{Evaluation results across different number of building blocks with IRM as training objective. The highest scores are highlighted in boldface.}
\label{tab7}
% \vspace*{0.1in}
\scalebox{1.2}{
\begin{tabular}{l||c||ccccc }
\hline
\textbf{Network}  & \# \textbf{Param.} & \textbf{PESQ} & \textbf{ESTOI} (\%) & \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} \\
\hline 
Noisy & - & 1.24 & 56.12 & 2.26  & 1.80  & 1.67 \\
\hline 
\hline
ResTCN-20+SA & 1.32M       
& 1.72 & 70.04 & 3.07 & 2.43 & 2.35  \\
ResTCN-20 & 1.05M       
& 1.70 & 68.92 & 3.05 & 2.41 & 2.33  \\
+TFA  & +1.36K     
& \textbf{1.82} & \textbf{72.17} & \textbf{3.22} & \textbf{2.51} & \textbf{2.47}  \\
\hline
ResTCN-30+SA & 1.78M   
& 1.75 & 70.45 & 3.11 & 2.47 & 2.39  \\
ResTCN-30 & 1.51M   
& 1.73 & 69.57 & 3.09 & 2.43 & 2.36  \\
+TFA  & +2.04K  
& \textbf{1.90} & \textbf{73.04} & \textbf{3.28} & \textbf{2.56} & \textbf{2.55}  \\
\hline
\hline
MHANet-4 & 3.29M   
& 1.75 & 70.58 & 3.12 & 2.45 & 2.39  \\
+TFA & +0.27K    
& \textbf{1.85} &\textbf{71.98} & \textbf{3.26} & \textbf{2.52} & \textbf{2.51}  \\
\hline
MHANet-6 & 4.86M
& 1.78 & 71.22 & 3.15 & 2.45 &  2.41 \\
+TFA & +0.41K
& \textbf{1.91} &\textbf{73.37} & \textbf{3.30} & \textbf{2.59} & \textbf{2.56}  \\
\hline
\hline
2S-SA-TCN & 2.87M
& 1.78 & 71.64 & 3.19 & 2.48 &  2.44 \\
+TFA & +3.2K
& \textbf{1.94} &\textbf{74.43} & \textbf{3.38} & \textbf{2.62} & \textbf{2.63}  \\
\hline
Conformer-5 & 6.97M
& 1.86 & 73.16 & 3.26 & 2.56 &  2.52 \\
+TFA & +0.68K
& \textbf{1.99} &\textbf{75.32} & \textbf{3.42} & \textbf{2.68} & \textbf{2.68}  \\
\hline
\end{tabular}}
\label{composite}
\vspace{-2.5em}
\end{table}

==> execution.tex <==
% \renewcommand\arraystretch{1.0}
\begin{table}[!htbp]
\centering
    \scriptsize
    \def\arraystretch{1.3}
    \setlength{\tabcolsep}{1.5pt}
\caption{Evaluation results of inference speed (RTF).}
% \vspace*{0.1in}
\scalebox{1.2}{
\begin{tabular}{l|c|c|c|c }
\hline
Network & ResTCN & ResTCN+TFA & MHANet & MHANet+TFA \\
\hline
RTF & $2.63\times\!10^{-4}$ & $3.14\times\!10^{-4}$ & $2.84\times\!10^{-4}$ & $3.02\times\!10^{-4}$ \\
\hline  
\end{tabular}}
\vspace{-1.0em}
\label{exet}
\end{table}

==> pesq.tex <==
\begin{table*}[!hb]
    \vspace{-1.0em}
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{3.3pt}
%   \captionsetup{justification=centering}
    \caption{
    Speech enhancement performance in terms of wide-band PESQ for different models and training targets.
    }
%   \vspace*{0.1in}
  \begin{tabular}{clc|ccccc|ccccc|ccccc|ccccc} 
   \hline
   \multirow{3}{*}{\textbf{Objective}} &
   \multirow{3}{*}{\textbf{Network}} &
   \multirow{3}{*}{\textbf{\# Params}}
%   \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\# params.}\\$\pmb{\times 10^{6}}$ \end{tabular}} 
   & \multicolumn{20}{c}{\textbf{SNR level (dB)}} \\
    \cline{4-23} & & & \multicolumn{5}{c|}{\textbf{Voice babble}} 
    & \multicolumn{5}{c|}{\textbf{Street music}} 
    & \multicolumn{5}{c|}{\textbf{F16}} 
    & \multicolumn{5}{c}{\textbf{Factory}}
    \\
    \cline{4-23}& & & {\bf-5}  & {\bf0}   & {\bf5}   & {\bf10}  & {\bf15} 
                    & {\bf-5}  & {\bf0}   & {\bf5}   & {\bf10}  & {\bf15} 
                    & {\bf-5}  & {\bf0}   & {\bf5}   & {\bf10}  & {\bf15}  
                    & {\bf-5}  & {\bf0}   & {\bf5}   & {\bf10}  & {\bf15} \\ 
    \hline
        
% Noisy & -- & 1.04 & 1.07 & 1.14 & 1.35 & 1.71 
%                   & 1.04 & 1.06 & 1.11 & 1.27 & 1.58 
%                   & 1.03 & 1.06 & 1.11 & 1.25 & 1.52 
%                   & 1.04 & 1.04 & 1.09 & 1.24 & 1.54 \\


- & Noisy & --    
& 1.07 & 1.12 & 1.23 & 1.47 & 1.89 
& 1.03 & 1.05 & 1.10 & 1.25 & 1.56 
& 1.04 & 1.06 & 1.11 & 1.27 & 1.58 
& 1.05 & 1.05 & 1.10 & 1.24 & 1.52 \\

\hline
\hline
\multirow{8}{*}{\rotatebox{360}{IRM}}
& ResTCN & 1.976M 
& 1.15 & 1.35 & 1.70 & 2.15 & 2.64 
& 1.12 & 1.27 & 1.56 & 1.97 & 2.43 
& 1.19 & 1.45 & 1.77 & 2.19 & 2.59 
& 1.11 & 1.29 & 1.56 & 1.99 & 2.37 \\
       

& +FA & +1.36K  
& 1.19 & 1.43 & 1.81 & 2.27 & 2.77
& 1.15 & 1.32 & 1.63 & 2.05 & 2.54 
& 1.26 & 1.52 & 1.91 & 2.34 & 2.76 
& 1.15 & 1.36 & 1.70 & 2.17 & 2.62\\ 

& +TA & +1.36K
& 1.16 & 1.41 & 1.82 & 2.30 & 2.78 
& 1.15 & 1.34 & 1.68 & 2.10 & 2.57 
& 1.26 & 1.53 & 1.88 & 2.30 & 2.70
& 1.17 & 1.38 & 1.72 & 2.16 & 2.54 \\

& +TFA & +2.72K
& \textbf{1.22} & \textbf{1.48} & \textbf{1.89} & \textbf{2.35} & \textbf{2.83}
& \textbf{1.18} & \textbf{1.39} & \textbf{1.75} & \textbf{2.16} & \textbf{2.60} 
& \textbf{1.32} & \textbf{1.61} & \textbf{1.97} & \textbf{2.39} & \textbf{2.79} 
& \textbf{1.21} & \textbf{1.41} & \textbf{1.80} & \textbf{2.24} & \textbf{2.65} \\ 

\cline{2-23}
& MHANet & 4.076M 
& 1.17 & 1.39 & 1.75 & 2.21 & 2.71 
& 1.13 & 1.30 & 1.59 & 1.97 & 2.43 
& 1.22 & 1.48 & 1.86 & 2.28 & 2.70 
& 1.11 & 1.27 & 1.56 & 1.96 & 2.38 \\

& +FA & +0.17K
& 1.17 & 1.40 & 1.78 & 2.25 & 2.71 
& 1.16 & 1.35 & 1.67 & 2.07 & 2.52 
& 1.26 & 1.51 & 1.89 & 2.35 & 2.80 
& 1.14 & 1.34 & 1.67 & 2.09 & 2.50 \\

& +TA & +0.17K
& 1.17 & 1.43 & 1.81 & 2.28 & 2.75 
& 1.16 & 1.36 & 1.67 & 2.08 & 2.52 
& 1.26 & 1.55 & 1.91 & 2.35 & 2.78 
& 1.15 & 1.38 & 1.70 & 2.12 & 2.50 \\

& +TFA & +0.34K
& \textbf{1.19} & \textbf{1.43} & \textbf{1.85} & \textbf{2.34} & \textbf{2.85} 
& \textbf{1.18} & \textbf{1.38} & \textbf{1.71} & \textbf{2.15} & \textbf{2.63} 
& \textbf{1.30} & \textbf{1.60} & \textbf{1.95} & \textbf{2.39} & \textbf{2.81} 
& \textbf{1.16} & \textbf{1.39} & \textbf{1.75} & \textbf{2.20} & \textbf{2.62} \\
\hline
\hline
    
\multirow{8}{*}{\rotatebox{360}{SMM}}
& ResTCN & 1.98M 
& 1.12 & 1.34 & 1.68 & 2.08 & 2.53 
& 1.11 & 1.27 & 1.51 & 1.90 & 2.36 
& 1.20 & 1.44 & 1.76 & 2.16 & 2.56 
& 1.11 & 1.27 & 1.55 & 1.96 & 2.36 \\

& +FA & +1.36K  
& 1.19 & 1.45 & 1.83 & 2.31 & 2.80 
& 1.15 & 1.34 & 1.66 & 2.08 & 2.55 
& 1.27 & 1.55 & 1.91 & 2.35 & 2.77 
& 1.15 & 1.34 & 1.68 & 2.14 & 2.59\\ 

& +TA & +1.36K
& 1.18 & 1.44 & 1.84 & 2.32 & 2.80 
& 1.15 & 1.35 & 1.70 & 2.12 & 2.58 
& 1.27 & 1.54 & 1.89 & 2.30 & 2.71
& 1.17 & 1.39 & 1.75 & 2.20 & 2.60 \\

& +TFA & +2.72K
& \textbf{1.21} & \textbf{1.51} & \textbf{1.93} & \textbf{2.39} & \textbf{2.86}
& \textbf{1.18} & \textbf{1.40} & \textbf{1.80} & \textbf{2.25} & \textbf{2.71} 
& \textbf{1.34} & \textbf{1.63} & \textbf{2.01} & \textbf{2.45} & \textbf{2.81} 
& \textbf{1.21} & \textbf{1.45} & \textbf{1.82} & \textbf{2.28} & \textbf{2.74} \\ 

\cline{2-23}
& MHANet & 4.076M 
& 1.16 & 1.39 & 1.75 & 2.22 & 2.71 
& 1.13 & 1.31 & 1.62 & 2.02 & 2.46 
& 1.24 & 1.50 & 1.84 & 2.26 & 2.70 
& 1.12 & 1.28 & 1.57 & 1.99 & 2.41 \\

& +FA & +0.17K
& 1.19 & 1.44 & 1.83 & 2.27 & 2.74 
& 1.17 & 1.37 & 1.70 & 2.13 & 2.59 
& 1.25 & 1.53 & 1.89 & 2.32 & 2.72 
& 1.14 & 1.34 & 1.66 & 2.10 & 2.52 \\

& +TA & +0.17K
& 1.19 & 1.46 & 1.86 & 2.35 & 2.83 
& 1.17 & 1.38 & 1.72 & 2.14 & 2.59 
& 1.28 & 1.59 & 1.92 & 2.33 & 2.76 
& 1.15 & 1.37 & 1.74 & 2.14 & 2.54 \\

& +TFA & +0.34K
& \textbf{1.21} & \textbf{1.49} & \textbf{1.89} & \textbf{2.37} & \textbf{2.85} 
& \textbf{1.19} & \textbf{1.41} & \textbf{1.75} & \textbf{2.19} & \textbf{2.64} 
& \textbf{1.30} & \textbf{1.61} & \textbf{2.00} & \textbf{2.45} & \textbf{2.84} 
& \textbf{1.17} & \textbf{1.42} & \textbf{1.78} & \textbf{2.21} & \textbf{2.64} \\
\hline
\hline
    
\multirow{8}{*}{\rotatebox{360}{PSM}}
& ResTCN & 1.98M 
& 1.17 & 1.39 & 1.74 & 2.25 & 2.79 
& 1.14 & 1.32 & 1.67 & 2.12 & 2.67 
& 1.27 & 1.55 & 1.92 & 2.35 & 2.80 
& 1.15 & 1.36 & 1.71 & 2.18 & 2.63 \\

& +FA & +1.36K  
& 1.21 & 1.43 & 1.86 & 2.37 & 2.86 
& 1.18 & 1.40 & 1.75 & 2.21 & 2.73 
& 1.30 & 1.59 & 2.01 & 2.52 & 2.97 
& 1.22 & 1.47 & 1.88 & 2.35 & 2.82\\ 

& +TA & +1.36K
& 1.17 & 1.45 & 1.89 & 2.41 & 2.91 
& 1.15 & 1.40 & 1.79 & 2.27 & 2.77 
& 1.32 & 1.64 & 2.01 & 2.49 & 2.91
& 1.21 & 1.49 & \textbf{1.89} & \textbf{2.36} & 2.80 \\

& +TFA & +2.72K
& \textbf{1.25} & \textbf{1.55} & \textbf{1.98} & \textbf{2.48} & \textbf{2.96}
& \textbf{1.22} & \textbf{1.47} & \textbf{1.87} & \textbf{2.32} & \textbf{2.79} 
& \textbf{1.35} & \textbf{1.66} & \textbf{2.11} & \textbf{2.59} & \textbf{3.01} 
& \textbf{1.25} & \textbf{1.50} & \textbf{1.89} & 2.34 & \textbf{2.86}\\ 

\cline{2-23}
& MHANet & 4.076M 
& 1.19 & 1.45 & 1.87 & 2.36 & 2.91 
& 1.18 & 1.40 & 1.74 & 2.18 & 2.66 
& 1.29 & 1.59 & 2.01 & 2.49 & 2.92 
& 1.16 & 1.37 & 1.74 & 2.26 & 2.69 \\

& +FA & +0.17K
& 1.19 & 1.45 & 1.87 & 2.38 & 2.90 
& 1.18 & 1.39 & 1.76 & 2.24 & 2.75 
& 1.31 & 1.61 & 2.04 & 2.54 & 2.97 
& 1.19 & 1.43 & 1.83 & 2.26 & 2.72 \\

& +TA & +0.17K
& 1.19 & 1.46 & 1.87 & 2.43 & \textbf{2.95} 
& 1.20 & 1.44 & 1.80 & 2.25 & 2.74 
& 1.32 & 1.63 & 2.03 & 2.53 & 3.01 
& 1.18 & 1.41 & 1.80 & 2.27 & \textbf{2.73} \\

& +TFA & +0.34K
& \textbf{1.20} & \textbf{1.48} & \textbf{1.92} & \textbf{2.45} & \textbf{2.95} 
& \textbf{1.21} & \textbf{1.46} & \textbf{1.85} & \textbf{2.31} & \textbf{2.80} 
& \textbf{1.34} & \textbf{1.66} & \textbf{2.09} & \textbf{2.60} & \textbf{3.03} 
& \textbf{1.23} & \textbf{1.50} & \textbf{1.90} & \textbf{2.37} & 2.72 \\
\hline
\hline

\multirow{8}{*}{\rotatebox{360}{Xi}}
& ResTCN & 1.98M 
& 1.16 & 1.38 & 1.72 & 2.25 & 2.77 
& 1.14 & 1.31 & 1.60 & 2.01 & 2.48 
& 1.26 & 1.54 & 1.92 & 2.33 & 2.77 
& 1.14 & 1.35 & 1.64 & 2.14 & 2.51 \\

& +FA & +1.36K  
& 1.21 & 1.43 & 1.82 & 2.37 & 2.88 
& 1.19 & 1.42 & 1.75 & 2.23 & 2.73 
& 1.31 & 1.60 & 2.04 & 2.52 & 2.96 
& 1.19 & 1.46 & 1.84 & 2.35 & 2.78\\ 

& +TA & +1.36K
& 1.19 & 1.46 & 1.86 & 2.42 & 2.92 
& 1.20 & 1.43 & 1.82 & 2.29 & 2.75 
& 1.31 & 1.60 & 1.96 & 2.40 & 2.88
& 1.21 & 1.47 & 1.85 & 2.28 & 2.73 \\

& +TFA & +2.72K
& \textbf{1.22} & \textbf{1.52} & \textbf{1.93} & \textbf{2.48} & \textbf{2.95}
& \textbf{1.24} & \textbf{1.48} & \textbf{1.86} & \textbf{2.32} & \textbf{2.77} 
& \textbf{1.38} & \textbf{1.69} & \textbf{2.10} & \textbf{2.60} & \textbf{3.01} 
& \textbf{1.26} & \textbf{1.53} & \textbf{1.93} & \textbf{2.43} & \textbf{2.83}\\ 

\cline{2-23}
& MHANet & 4.076M 
& 1.18 & 1.43 & 1.77 & 2.30 & 2.84 
& 1.18 & 1.38 & 1.71 & 2.16 & 2.67 
& 1.28 & 1.60 & 2.06 & 2.53 & 2.98 
& 1.16 & 1.38 & 1.78 & 2.25 & 2.66 \\

& +FA & +0.17K
& 1.19 & 1.42 & 1.78 & 2.36 & 2.89 
& 1.20 & 1.42 & 1.75 & 2.24 & \textbf{2.74} 
& 1.29 & 1.61 & 2.03 & 2.53 & 2.99 
& 1.19 & 1.45 & 1.80 & 2.29 & 2.69 \\

& +TA & +0.17K
& 1.06 & \textbf{1.45} & 1.80 & 2.39 & 2.91 
& 1.19 & 1.41 & 1.76 & 2.16 & 2.59 
& 1.31 & 1.62 & 2.03 & 2.52 & 2.96 
& 1.19 & 1.44 & 1.82 & 2.24 & 2.67 \\

& +TFA & +0.34K
& \textbf{1.20} & \textbf{1.45} & \textbf{1.85} & \textbf{2.40} & \textbf{2.93} 
& \textbf{1.21} & \textbf{1.43} & \textbf{1.82} & \textbf{2.29} & 2.73 
& \textbf{1.34} & \textbf{1.67} & \textbf{2.07} & \textbf{2.56} & \textbf{3.00} 
& \textbf{1.21} & \textbf{1.46} & \textbf{1.88} & \textbf{2.32} & \textbf{2.71} \\
\hline
\end{tabular}
\label{tab:pesq}
\end{table*}

==> results_dB.tex <==
\begin{table*}[!t]
\centering
    % \scriptsize
    % \footnotesize
    \small
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.3pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
\caption{\textcolor{blue}{The evaluation results on noisy conditions, where each audio recording is mixed with a random segment from a babble noise recording at 0 dB, 5 dB, and 10 dB SNR levels, respectively.}}
% \vspace*{-0.5em}
% \scalebox{1}{
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
% \toprule
\toprule[1.5pt]
% \hline
% Task & Acoustic Scene & \multicolumn{2}{c|}{Music Genre} & \multicolumn{2}{c|}{Speech Emotion} & \multicolumn{2}{c|}{keyword Spotting} & Speaker Id. \\
% \hline
\multirow{2}{*}{Method}& \multirow{2}{*}{SNR (dB)} & \multicolumn{2}{c|}{ESC-50} & \multicolumn{2}{c|}{GTZAN} &  \multicolumn{2}{c|}{FMA-Small} & \multicolumn{2}{c|}{CREMA-D} & \multicolumn{2}{c|}{SPC-V1} & \multicolumn{2}{c}{SPC-V2} \\
% \hline
\cline{3-14}
 & & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
% \hline
% Segment & -- & -- & -- & -- & -- & -- & -- & 1 s & 3 s \\
% \hline
% \hline
% LEAF & \multirow{3}{*}{MNet-V2} &
% \textcolor{black}{64.80} & \textcolor{black}{88.00} & \textcolor{red}{38.18} & \textcolor{red}{88.27} & \textcolor{red}{37.50} & \textcolor{red}{88.50} & \textcolor{red}{34.43} & \textcolor{red}{96.07} & \textcolor{red}{61.61} & \textcolor{red}{89.34} & \textcolor{red}{68.44} & \textcolor{red}{89.22} \\

% Ada-FE & & 
% \textbf{\textcolor{black}{65.30}}  & \textcolor{black}{88.05} & \textbf{\textcolor{red}{44.32}}  & \textcolor{red}{90.34} & \textcolor{red}{38.38} & \textcolor{red}{88.13} & \textcolor{red}{28.89} & \textcolor{red}{95.49} & \textcolor{red}{62.94}  &  \textcolor{red}{85.33}  & \textcolor{red}{59.16} & \textcolor{red}{81.52} \\

% Ada-FE-S-F & & 
% \textcolor{black}{64.55}  & \textbf{\textcolor{black}{88.40}} & \textcolor{red}{45.51}  & \textcolor{red}{91.51} & \textcolor{red}{35.38} & \textcolor{red}{89.50} & \textcolor{red}{32.11} & \textcolor{red}{94.97} & \textcolor{red}{61.03} & \textcolor{red}{84.94} & \textcolor{red}{61.93} & \textcolor{red}{84.12} \\
\hline
\hline

Fixed-Q & \multirow{2}{*}{0} & 
\textcolor{black}{64.85}  & \textcolor{black}{88.25} & \textcolor{blue}{28.97}  & \textcolor{blue}{70.00} & \textcolor{blue}{25.37} & \textcolor{blue}{80.50} & \textcolor{blue}{21.02} & \textcolor{blue}{94.58} & \textcolor{blue}{46.51} & \textcolor{blue}{73.39} & \textcolor{blue}{39.34} & \textcolor{blue}{64.96} \\

% Ada-FE &  & 
% \textcolor{black}{59.60} & \textcolor{black}{86.20} & \textcolor{blue}{48.23} & \textcolor{blue}{90.58} & \textcolor{black}{39.63} & \textcolor{black}{90.25} & \textcolor{black}{28.69} & \textcolor{black}{95.68} & \textcolor{black}{77.71} & \textcolor{black}{92.64} & \textcolor{black}{73.36} & \textcolor{black}{90.34} \\

% CREMAD Fixed E93

Ada-FE &  & 
\textcolor{black}{57.95} & \textcolor{black}{85.65} & \textcolor{blue}{31.72} & \textcolor{blue}{76.55} & \textcolor{blue}{26.50} & \textcolor{blue}{80.63} & \textcolor{blue}{25.98} & \textcolor{blue}{94.81} & \textcolor{blue}{48.63} & \textcolor{blue}{75.29} & \textcolor{blue}{41.42} & \textcolor{blue}{67.56} \\

\hline

Fixed-Q & \multirow{2}{*}{5} & 
\textcolor{black}{64.85}  & \textcolor{black}{88.25} & \textcolor{blue}{41.03}  & \textcolor{blue}{80.34} & \textcolor{blue}{30.50} & \textcolor{blue}{86.75} & \textcolor{blue}{24.37} & \textcolor{blue}{95.42} & \textcolor{blue}{67.69} & \textcolor{blue}{88.27} & \textcolor{blue}{62.21} & \textcolor{blue}{82.85} \\


Ada-FE &  & 
\textcolor{black}{59.60} & \textcolor{black}{86.20} & \textcolor{blue}{44.83} & \textcolor{blue}{84.14} & \textcolor{blue}{33.13} & \textcolor{blue}{84.75} & \textcolor{blue}{27.98} & \textcolor{blue}{95.81} & \textcolor{blue}{70.14} & \textcolor{blue}{89.37} & \textcolor{blue}{62.67} & \textcolor{blue}{84.22} \\

% Ada-FE-S-F &  & 
% \textcolor{black}{57.95} & \textcolor{black}{85.65} & \textcolor{black}{47.59} & \textcolor{black}{90.23} & \textcolor{black}{44.13} & \textcolor{black}{91.63} & \textcolor{black}{37.20} & \textcolor{black}{95.55} & \textcolor{black}{77.65} & \textcolor{black}{92.29} & \textcolor{black}{74.32} & \textcolor{black}{90.98} \\

\hline

Fixed-Q & \multirow{2}{*}{10} & 
\textcolor{black}{64.85}  & \textcolor{black}{88.25} & \textcolor{blue}{47.93}  & \textcolor{blue}{88.28} & \textcolor{blue}{36.50} & \textcolor{blue}{88.25} & \textcolor{blue}{31.21} & \textcolor{blue}{96.26} & \textcolor{blue}{81.31} & \textcolor{blue}{94.03} & \textcolor{blue}{75.93} & \textcolor{blue}{91.26} \\


Ada-FE &  & 
\textcolor{black}{59.60} & \textcolor{black}{86.20} & \textcolor{blue}{51.03} & \textcolor{blue}{90.69} & \textcolor{blue}{39.50} & \textcolor{blue}{88.38} & \textcolor{blue}{34.36} & \textcolor{blue}{96.39} & \textcolor{blue}{82.40} & \textcolor{blue}{94.56} & \textcolor{blue}{77.32} & \textcolor{blue}{92.43} \\

% Ada-FE-S-F &  & 
% \textcolor{black}{57.95} & \textcolor{black}{85.65} & \textcolor{blue}{47.59} & \textcolor{blue}{90.23} & \textcolor{blue}{44.13} & \textcolor{blue}{91.63} & \textcolor{blue}{37.20} & \textcolor{blue}{95.55} & \textcolor{blue}{77.65} & \textcolor{blue}{92.29} & \textcolor{blue}{74.32} & \textcolor{blue}{90.98} \\

\toprule[1.5pt]
% \toprule
% \hline
% \rowcolor{orange!20} \,\,\,\,\, Fixed Gabor filter+AFC-Energy+FM & -- & -- & 54.14 & 95.52 & 45.38 & 93.63 & 59.78 & 98.84 & 91.92 & 98.19 \\
\end{tabular}
\label{ablation}
% }
\end{table*}

==> reverb.tex <==
\begin{table*}[!t]
\centering
    % \scriptsize
    % \footnotesize
    \small
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.3pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
\caption{\textcolor{blue}{The results on noisy acoustic conditions, where each clean clip is mixed with the noise in a random SNR level selected from 5 to 15 dB.}}
% \vspace*{-0.5em}
% \scalebox{1}{
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
\toprule
% \hline
% Task & Acoustic Scene & \multicolumn{2}{c|}{Music Genre} & \multicolumn{2}{c|}{Speech Emotion} & \multicolumn{2}{c|}{keyword Spotting} & Speaker Id. \\
% \hline
Task & \multirow{2}{*}{Back-end} & \multicolumn{2}{c|}{ESC-50} & \multicolumn{2}{c|}{GTZAN} &  \multicolumn{2}{c|}{FMA-Small} & \multicolumn{2}{c|}{CREMA-D} & \multicolumn{2}{c|}{SPC-V1} & \multicolumn{2}{c}{SPC-V2} \\
% \hline
\cline{3-14}
Accuracy & & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
% \hline
% Segment & -- & -- & -- & -- & -- & -- & -- & 1 s & 3 s \\
\hline
\hline
LEAF & \multirow{3}{*}{MNet-V2} &
\textcolor{black}{64.80} & \textcolor{black}{88.00} & \textcolor{red}{38.18} & \textcolor{red}{88.27} & \textcolor{red}{37.50} & \textcolor{red}{88.50} & \textcolor{red}{34.43} & \textcolor{red}{96.07} & \textcolor{red}{61.61} & \textcolor{red}{89.34} & \textcolor{red}{68.44} & \textcolor{red}{89.22} \\

Ada-FE & & 
\textbf{\textcolor{black}{65.30}}  & \textcolor{black}{88.05} & \textbf{\textcolor{red}{44.32}}  & \textcolor{red}{90.34} & \textcolor{red}{38.38} & \textcolor{red}{88.13} & \textcolor{red}{28.89} & \textcolor{red}{95.49} & \textcolor{red}{62.94}  &  \textcolor{red}{85.33}  & \textcolor{red}{59.16} & \textcolor{red}{81.52} \\

Ada-FE-S-F & & 
\textcolor{black}{64.55}  & \textbf{\textcolor{black}{88.40}} & \textcolor{red}{45.51}  & \textcolor{red}{91.51} & \textcolor{red}{35.38} & \textcolor{red}{89.50} & \textcolor{red}{32.11} & \textcolor{red}{94.97} & \textcolor{red}{61.03} & \textcolor{red}{84.94} & \textcolor{red}{61.93} & \textcolor{red}{84.12} \\
\hline

LEAF & \multirow{3}{*}{ENet-B0} & 
\textcolor{black}{64.85}  & \textcolor{black}{88.25} & \textcolor{red}{45.73}  & \textcolor{red}{90.17} & \textcolor{red}{37.63} & \textcolor{red}{91.00} & \textcolor{red}{46.23} & \textcolor{red}{97.36} & \textcolor{red}{81.84} & \textcolor{red}{94.66} & \textcolor{red}{81.06} & \textcolor{red}{94.09} \\

Ada-FE &  & 
\textcolor{black}{59.60} & \textcolor{black}{86.20} & \textcolor{red}{48.23} & \textcolor{red}{90.58} & \textcolor{red}{39.63} & \textcolor{red}{90.25} & \textcolor{red}{28.69} & \textcolor{red}{95.68} & \textcolor{red}{77.71} & \textcolor{red}{92.64} & \textcolor{red}{73.36} & \textcolor{red}{90.34} \\

Ada-FE-S-F &  & 
\textcolor{black}{57.95} & \textcolor{black}{85.65} & \textcolor{red}{47.59} & \textcolor{red}{90.23} & \textcolor{red}{44.13} & \textcolor{red}{91.63} & \textcolor{red}{37.20} & \textcolor{red}{95.55} & \textcolor{red}{77.65} & \textcolor{red}{92.29} & \textcolor{red}{74.32} & \textcolor{red}{90.98} \\

\toprule
% \hline
% \rowcolor{orange!20} \,\,\,\,\, Fixed Gabor filter+AFC-Energy+FM & -- & -- & 54.14 & 95.52 & 45.38 & 93.63 & 59.78 & 98.84 & 91.92 & 98.19 \\
\end{tabular}
\label{ablation}
% }
\end{table*}

==> stoi.tex <==
\begin{table*}[!ht]
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.45pt}
%   \captionsetup{justification=centering}
    \caption{
    Speech enhancement performance in terms of ESTOI (\%) metric for different models and training targets.
    }
%   \vspace*{0.15in}
  \begin{tabular}{clc|ccccc|ccccc|ccccc|ccccc} 
  \hline
   \multirow{3}{*}{\textbf{Objective}} &
   \multirow{3}{*}{\textbf{Network}} &
   \multirow{3}{*}{\textbf{\# Params}}
%   \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\# params.}\\$\pmb{\times 10^{6}}$ \end{tabular}} 
   & \multicolumn{20}{c}{\textbf{SNR level (dB)}} \\
    \cline{4-23} & & & \multicolumn{5}{c|}{\textbf{Voice babble}} 
    & \multicolumn{5}{c|}{\textbf{Street music}} 
    & \multicolumn{5}{c|}{\textbf{F16}} 
    & \multicolumn{5}{c}{\textbf{Factory}}
    \\
    \cline{4-23}& & & {\bf-5} & {\bf0} & {\bf5} & {\bf10} & {\bf15} 
                    & {\bf-5} & {\bf0} & {\bf5} & {\bf10} & {\bf15} 
                    & {\bf-5} & {\bf0} & {\bf5} & {\bf10} & {\bf15} 
                    & {\bf-5} & {\bf0} & {\bf5} & {\bf10} & {\bf15} \\ 
    \hline
        
% Noisy & -- & 1.04 & 1.07 & 1.14 & 1.35 & 1.71 
%                   & 1.04 & 1.06 & 1.11 & 1.27 & 1.58 
%                   & 1.03 & 1.06 & 1.11 & 1.25 & 1.52 
%                   & 1.04 & 1.04 & 1.09 & 1.24 & 1.54 \\

- & Noisy & -- 
& 28.76 & 44.42 & 60.67 & 74.97 & 85.37 
& 30.39 & 44.03 & 58.15 & 71.13 & 81.80 
& 27.45 & 41.89 & 56.70 & 70.27 & 81.30 
& 25.03 & 38.45 & 53.30 & 68.09 & 80.42 \\

\hline
\hline
\multirow{8}{*}{\rotatebox{360}{IRM}}
& ResTCN & 1.98M 
& 39.22 & 58.59 & 74.23 & 84.70 & 90.89 
& 45.06 & 61.84 & 74.41 & 83.12 & 89.00 
& 46.48 & 62.90 & 75.21 & 83.98 & 89.94 
& 39.38 & 57.62 & 71.88 & 82.04 & 88.59 \\

& +FA & +1.36K  
& 42.58 & 61.54 & 76.28 & 85.53 & 91.38 
& 47.00 & 62.73 & 75.25 & 83.81 & 89.56 
& 49.51 & 64.79 & 76.59 & 85.16 & 90.51 
& 41.96 & 59.65 & 73.83 & 83.46 & 89.59 \\ 

& +TA & +1.36K
& 42.35 & 61.90 & 76.61 & 85.99 & 91.52 
& 48.67 & 64.83 & 76.21 & 84.26 & 89.70 
& 52.21 & 66.89 & 77.64 & 85.46 & 90.82
& 44.43 & 61.84 & 74.84 & 83.97 & 89.84 \\

& +TFA & +2.72K
& \textbf{44.72} & \textbf{63.56} & \textbf{77.79} & \textbf{86.39} & \textbf{91.80}
& \textbf{50.40} & \textbf{66.01} & \textbf{77.23} & \textbf{84.78} & \textbf{89.96} 
& \textbf{53.97} & \textbf{67.97} & \textbf{78.50} & \textbf{86.37} & \textbf{91.36} 
& \textbf{46.22} & \textbf{62.88} & \textbf{75.86} & \textbf{84.72} & \textbf{90.48} \\ 

% \cmidrule{2-23}
\cline{2-23}
& MHANet & 4.076M 
& 42.83 & 61.36 & 75.47 & 85.27 & 91.28 
& 47.38 & 63.13 & 75.49 & 83.81 & 89.56 
& 47.70 & 64.36 & 76.68 & 85.00 & 90.55 
& 40.46 & 57.74 & 72.34 & 82.20 & 88.60 \\

& +FA & +0.2K
& 42.24 & 61.15 & 75.96 & 85.67 & 91.38 
& 48.64 & 64.35 & 76.31 & 84.39 & 89.96 
& 50.24 & 65.58 & 77.33 & 85.63 & 91.08 
& 41.45 & 59.27 & 73.65 & 83.22 & 89.35 \\

& +TA & +0.2K
& 42.95 & 62.53 & 76.65 & 86.02 & 91.69 
& 48.56 & 64.35 & 76.03 & 84.00 & 89.68 
& 50.27 & 66.23 & 77.73 & 85.69 & 91.16 
& 43.10 & 60.64 & 74.36 & 83.50 & 89.41 \\

& +TFA & +0.41K
& \textbf{43.31} & \textbf{62.58} & \textbf{77.47} & \textbf{86.43} & \textbf{91.92} 
& \textbf{49.16} & \textbf{64.75} & \textbf{76.60} & \textbf{84.65} & \textbf{90.18} 
& \textbf{52.08} & \textbf{66.99} & \textbf{78.10} & \textbf{86.07} & \textbf{91.29} 
& \textbf{44.67} & \textbf{62.02} & \textbf{75.18} & \textbf{83.96} & \textbf{89.91} \\
% \bottomrule
% \bottomrule
\hline
\hline
    
\multirow{8}{*}{\rotatebox{360}{SMM}}
& ResTCN & 1.98M 
& 38.18 & 56.88 & 72.04 & 82.33 & 89.12 
& 43.17 & 59.59 & 72.47 & 81.69 & 88.09 
& 45.97 & 62.51 & 74.82 & 83.67 & 89.76 
& 38.62 & 56.37 & 71.37 & 81.47 & 88.14 \\

& +FA & +1.36K  
& 41.65 & 62.27 & 76.17 & 85.64 & 91.35 
& 46.84 & 63.20 & 75.60 & 83.95 & 89.64 
& 50.29 & 65.37 & 76.66 & 85.07 & 90.52 
& 41.95 & 59.49 & 73.62 & 83.19 & 89.43 \\ 

& +TA & +1.36K
& 42.48 & 62.25 & 76.93 & 85.95 & 91.37 
& 48.34 & 64.85 & 76.42 & 84.19 & 89.65 
& 51.61 & 66.90 & 77.79 & 85.14 & 90.63
& 44.50 & 61.69 & 75.16 & 84.28 & 89.92 \\

& +TFA & +2.72K
& \textbf{43.74} & \textbf{64.28} & \textbf{78.47} & \textbf{86.57} & \textbf{91.73}
& \textbf{48.96} & \textbf{65.06} & \textbf{77.55} & \textbf{85.18} & \textbf{90.09} 
& \textbf{54.15} & \textbf{68.48} & \textbf{78.65} & \textbf{86.13} & \textbf{91.01} 
& \textbf{47.57} & \textbf{64.12} & \textbf{76.39} & \textbf{84.50} & \textbf{90.12} \\ 

% \cmidrule{2-23}
\cline{2-23}
& MHA & 4.076M 
& 41.87 & 61.38 & 75.79 & 85.34 & 91.26 
& 47.31 & 63.44 & 75.83 & 83.98 & 89.70 
& 49.71 & 65.27 & 77.07 & 85.25 & 90.88 
& 41.66 & 59.31 & 73.10 & 82.83 & 89.00 \\

& +FA & +0.2K
& 43.20 & 62.25 & 76.62 & 85.99 & 91.71 
& 48.34 & 64.02 & 76.46 & 84.76 & 90.18 
& 50.28 & 65.82 & 77.58 & 85.73 & 91.13 
& 41.68 & 59.68 & 73.63 & 83.39 & 89.56 \\

& +TA & +0.2K
& 43.11 & 62.81 & 77.00 & \textbf{86.45} & \textbf{91.99} 
& 49.49 & 65.22 & 76.80 & 84.83 & 90.19 
& 51.63 & 67.40 & 78.38 & 85.85 & 91.37 
& 44.07 & 61.07 & 74.85 & 83.54 & 89.63 \\

& +TFA & +0.41K
& \textbf{44.70} & \textbf{64.06} & \textbf{77.58} & 86.42 & 91.83 
& \textbf{50.47} & \textbf{65.92} & \textbf{77.58} & \textbf{85.19} & \textbf{90.35} 
& \textbf{52.97} & \textbf{67.60} & \textbf{78.66} & \textbf{86.33} & \textbf{91.71} 
& \textbf{44.88} & \textbf{61.81} & \textbf{75.55} & \textbf{84.27} & \textbf{90.23} \\
% \bottomrule
% \bottomrule
\hline
\hline
    
\multirow{8}{*}{\rotatebox{360}{PSM}}
& ResTCN & 1.98M 
& 40.46 & 59.53 & 74.71 & 85.03 & 90.92 
& 45.69 & 61.95 & 75.31 & 83.96 & 89.67 
& 46.66 & 63.14 & 75.45 & 84.16 & 89.91 
& 38.22 & 57.17 & 72.41 & 82.48 & 88.85 \\

& +FA & +1.36K  
& 41.41 & 60.89 & 76.18 & 85.67 & 91.34 
& 46.43 & 62.95 & 75.44 & 83.92 & 89.64 
& 50.22 & 66.09 & 77.58 & 86.02 & 91.06 
& 41.58 & 59.60 & 74.30 & 83.66 & 89.77 \\ 

& +TA & +1.36K
& 41.28 & 61.08 & 76.64 & 86.05 & 91.61 
& 47.03 & 63.73 & 76.22 & 84.49 & 90.02 
& 51.39 & 66.82 & 77.75 & 85.53 & 90.97
& 43.11 & 61.36 & 75.36 & 84.31 & 90.20 \\

& +TFA & +2.72K
& \textbf{45.44} & \textbf{64.63} & \textbf{78.23} & \textbf{86.81} & \textbf{92.10}
& \textbf{49.01} & \textbf{65.22} & \textbf{76.85} & \textbf{84.79} & \textbf{90.17} 
& \textbf{53.66} & \textbf{68.30} & \textbf{78.64} & \textbf{86.43} & \textbf{91.49} 
& \textbf{45.90} & \textbf{62.15} & \textbf{75.53} & \textbf{84.57} & \textbf{90.46} \\ 

% \cmidrule{2-23}
\cline{2-23}
& MHANet & 4.076M 
& 41.99 & 61.78 & 76.37 & 85.86 & 91.59 
& 46.78 & 63.11 & 75.89 & 84.30 & 89.83 
& 49.27 & 65.71 & 78.01 & 85.94 & 91.09 
& 40.63 & 58.99 & 73.62 & 83.38 & 89.49 \\

& +FA & +0.2K
& 41.84 & 61.56 & 76.31 & 85.83 & 91.51 
& 47.79 & 63.92 & 76.06 & 84.57 & 90.11 
& 48.48 & 65.53 & 78.88 & 85.88 & 91.06 
& 41.06 & 58.98 & 73.73 & 83.39 & 89.50 \\

& +TA & +0.2K
& 42.49 & 62.32 & \textbf{77.22} & 86.53 & 91.87 
& 48.07 & 64.41 & 76.30 & 84.47 & 90.12 
& 50.73 & 67.15 & 78.48 & 86.17 & 91.37 
& 42.46 & 60.37 & 74.40 & 83.72 & 89.63 \\

& +TFA & +0.41K
& \textbf{42.76} & \textbf{62.35} & 77.20 & \textbf{86.65} & \textbf{91.96} 
& \textbf{48.60} & \textbf{64.57} & \textbf{76.74} & \textbf{84.84} & \textbf{90.33} 
& \textbf{51.97} & \textbf{67.19} & \textbf{78.62} & \textbf{86.65} & \textbf{91.60} 
& \textbf{43.74} & \textbf{61.43} & \textbf{74.99} & \textbf{84.27} & \textbf{90.25} \\
% \bottomrule
% \bottomrule
\hline
\hline

\multirow{8}{*}{\rotatebox{360}{Xi}}
& ResTCN & 1.98M 
& 38.43 & 57.56 & 73.29 & 84.47 & 90.61 
& 42.79 & 60.15 & 73.74 & 82.91 & 88.81 
& 46.90 & 63.07 & 75.39 & 83.76 & 89.78 
& 37.06 & 56.63 & 71.88 & 82.30 & 88.69 \\

& +FA & +1.36K  
& 40.53 & 60.20 & 75.71 & 85.57 & 91.17 
& 44.80 & 62.31 & 75.39 & 83.95 & 89.63 
& 49.41 & 64.89 & 76.92 & 85.19 & 90.70 
& 40.21 & 59.16 & 73.28 & 82.97 & 89.10 \\ 

& +TA & +1.36K
& 42.05 & 61.59 & 76.18 & 85.75 & 91.44 
& 46.85 & 63.28 & 76.04 & 84.23 & 89.81 
& 50.92 & 66.32 & 77.41 & 84.87 & 90.64
& 42.23 & 60.25 & 73.81 & 83.14 & 89.30 \\

& +TFA & +2.72K
& \textbf{42.78} & \textbf{63.58} & \textbf{77.47} & \textbf{86.59} & \textbf{91.85}
& \textbf{48.83} & \textbf{64.97} & \textbf{76.71} & \textbf{84.51} & \textbf{89.98} 
& \textbf{54.09} & \textbf{68.41} & \textbf{78.73} & \textbf{86.33} & \textbf{91.44} 
& \textbf{45.11} & \textbf{62.39} & \textbf{74.66} & \textbf{84.01} & \textbf{90.14} \\ 

\cline{2-23}
& MHA & 4.076M 
& 40.44 & 60.80 & 75.26 & 85.23 & 91.21 
& 45.71 & 62.86 & 75.34 & 83.83 & 89.71 
& 48.48 & 65.65 & 77.68 & 85.53 & 90.91 
& 38.99 & 58.05 & 73.10 & 83.13 & 89.31 \\

& +FA & +0.17K
& 39.80 & 60.26 & 75.37 & 85.69 & 91.48 
& 45.24 & 63.20 & 75.95 & 84.27 & 89.88 
& 48.69 & 65.19 & 77.21 & 85.50 & 91.03 
& 39.92 & 58.74 & 73.64 & 83.33 & 89.37 \\

& +TA & +0.17K
& 41.24 & \textbf{61.84} & 76.24 & 85.79 & 91.49 
& 45.74 & 62.84 & 76.02 & 84.00 & 89.51 
& 49.37 & 66.17 & \textbf{77.96} & 85.66 & 90.97 
& 41.31 & 59.45 & 73.54 & 83.20 & 89.39 \\

& +TFA & +0.34K
& \textbf{41.25} & 61.22 & \textbf{76.46} & \textbf{85.93} & \textbf{91.55} 
& \textbf{46.45} & \textbf{63.63} & \textbf{76.31} & \textbf{84.50} & \textbf{89.92} 
& \textbf{50.51} & \textbf{66.51} & 77.94 & \textbf{85.78} & \textbf{91.22} 
& \textbf{43.39} & \textbf{60.82} & \textbf{74.53} & \textbf{83.69} & \textbf{89.64} \\
\hline
\end{tabular}
\vspace{-1.2em}
\label{tab:estoi}
\end{table*}

==> wer.tex <==
\begin{table}[!hbtp]
    \centering
    \scriptsize
    \def\arraystretch{0.965}
    \setlength{\tabcolsep}{4pt}
    % \footnotesize	
    \caption{Average WER\% results for each SNR condition and the WER\% scores averaged over all noisy conditions. The lowest WER\% scores are highlighted in boldface.}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||cccccc@{}}
        \hline
        &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}} & \\  
        \cline{3-7}
        Objective & Network & -5 & 0 & 5 & 10 & 15 & Avg \\
        \hline
        - & Noisy & 90.07 & 61.98 & 31.48 & 19.39 & 12.54 & 43.09 \\
        \hline
        \hline
        \multirow{8}{*}{IRM}
        & ResTCN & 84.57 & 58.78 & 29.79 & 18.30 & 11.35 & 40.55 \\
        & +FA & 81.80 & 53.63 & 27.50 & 15.62 & 9.18 & 37.55 \\
        & +TA & 82.33 & 49.50 & 26.93 & 14.23 & 8.56 & 36.31\\
        & +TFA & \textbf{75.49} & \textbf{48.48} & \textbf{25.37} & \textbf{12.91} & \textbf{8.50}& \textbf{34.15}\\
        \cline{2-8}
        & MHANet & 84.46 & 53.59 & 28.32 & 17.30 & 11.60 & 39.05\\
        & +FA & 83.33 & 50.02 & 26.46 & 16.50 & 9.18 & 37.14\\
        & +TA & 81.79 & 50.20 & 26.82 & 16.94 & 10.05 & 37.16\\
        & +TFA & \textbf{79.58} & \textbf{48.48} & \textbf{26.44} & \textbf{14.87} & \textbf{9.13 }& \textbf{35.70}\\
        \hline
        \hline
        
        \multirow{8}{*}{SMM}
        & ResTCN & 86.82 & 56.86 & 30.53 & 20.00 & 11.32 & 41.10 \\
        & +FA & 80.67 & 52.95 & 29.63 & 17.58 & 10.27 & 38.22 \\
        & +TA & 82.82 & 51.59 & 27.75 & 16.93 & 9.36 & 37.69 \\
        & +TFA & \textbf{79.77} & \textbf{46.88} & \textbf{26.67} & \textbf{13.61} & \textbf{9.00 }& \textbf{35.19}\\
        \cline{2-8}
        & MHANet & 84.22 & 53.06 & 27.58 & 18.14 & 11.60 & 38.92\\
        & +FA & 83.15 & 50.29 & 26.81 & 16.12 & 9.49 & 37.17\\
        & +TA & 82.35 & 51.47 & \textbf{25.71} & 17.37 & \textbf{8.60 }& 37.10\\
        & +TFA & \textbf{81.21} & \textbf{50.21} & 27.06 & \textbf{14.48} & \textbf{8.60 }& \textbf{36.33} \\
        \hline
        \hline
        
        \multirow{8}{*}{PSM}
        & ResTCN & 84.55 & 58.02 & 32.52 & 18.17 & 10.33 & 40.72\\
        & +FA & 80.74 & 56.56 & 27.23 & 17.16 & 9.65 & 38.37\\
        & +TA & 84.44 & 52.07 & 27.63 & \textbf{12.89} & 9.23 & 37.25\\
        & +TFA & \textbf{80.64} & \textbf{46.31} & \textbf{26.59} & 15.15 & \textbf{8.47} & \textbf{35.43}\\
        \cline{2-8}
        & MHANet & 84.83 & 52.78 & 28.26 & 18.76 & 11.56 & 39.24\\
        & +FA & 84.71 & 54.71 & 27.60 & 17.45 & \textbf{8.56 }& 38.60\\
        & +TA & 84.04 & 52.65 & \textbf{26.65} & 17.04 & 8.62 & 37.81\\
        & +TFA & \textbf{80.30} & \textbf{50.79} & 27.98 & \textbf{15.64} & 10.75 & \textbf{37.09}\\
        \hline
        \hline
        
        \multirow{8}{*}{Xi}
        & ResTCN & 88.99 & 58.92 & 32.99 & 17.83 & 10.82 & 41.91\\
        & +FA & 83.98 & 53.92 & 28.00 & 18.46 & 10.56 & 38.98\\
        & +TA & 82.79 & 51.14 & 28.90 & \textbf{14.76} & 11.59 & 37.83\\
        & +TFA & \textbf{80.75} & \textbf{47.23} & \textbf{25.57} & 17.45 & \textbf{9.43} & \textbf{36.09}\\
        \cline{2-8}
        & MHANet & 85.58 & 57.62 & 30.02 & 19.73 & 10.97 & 40.83\\
        & +FA & 84.95 & \textbf{52.27} & 29.27 & 17.71 & \textbf{9.95} & 38.83\\
        & +TA & \textbf{82.44} & 54.44 & \textbf{27.35} & 18.79 & 11.17 & 38.84\\
        & +TFA & 84.47 & 52.93 & 28.79 & \textbf{17.28} & \textbf{9.95} & \textbf{38.68}\\
        \hline
        
\end{tabular}
\label{tab:wer}
\vspace{-1.5em}
\end{table}
